Visual Imitation Learning with Patch Rewards

Visual imitation learning enables reinforcement learning agents to learn to behave from expert visual demonstrations such as videos or image sequences, without explicit, well-defined rewards. Previous research either adopted supervised learning techniques or induce simple and coarse scalar rewards from pixels, neglecting the dense information contained in the image demonstrations. In this work, we propose to measure the expertise of various local regions of image samples, or called \textit{patches}, and recover multi-dimensional \textit{patch rewards} accordingly. Patch reward is a more precise rewarding characterization that serves as a fine-grained expertise measurement and visual explainability tool. Specifically, we present Adversarial Imitation Learning with Patch Rewards (PatchAIL), which employs a patch-based discriminator to measure the expertise of different local parts from given images and provide patch rewards. The patch-based knowledge is also used to regularize the aggregated reward and stabilize the training. We evaluate our method on DeepMind Control Suite and Atari tasks. The experiment results have demonstrated that PatchAIL outperforms baseline methods and provides valuable interpretations for visual demonstrations.

==> conclusion.tex <==
\section{Conclusion}
We proposed PatchAIL, an intuitive and principled learning framework for efficient visual imitation learning (VIL). PatchAIL offers explainable patch-level rewards, which measure the expertise of various parts of given images and use this information to regularize the aggregated reward and stabilize the training, in place of less informative scalar rewards. We evaluate our method on the widely-used pixel-based benchmark DeepMind Control Suite. The results indicate that PatchAIL supports efficient training that outperforms baseline methods and provides valuable interpretations for VIL. We think that the proposed patch reward is a crucial method for utilizing the wealth of information contained in image observations, and that there is still a great potential for leveraging the patch-level information to enhance visual reinforcement learning and visual imitation learning.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
% Reinforcement learning (RL) has gained huge success in various domains including board games (e.g., Go~\citep{silver2017masteringgo}, chess~\citep{silver2017mastering}), card games (e.g., Texas Hold'em~\citep{brown2018superhuman}, 
% Mahjong~\citep{li2020suphx},  DouDizhu~\citep{guan2022perfectdou}) and video games (e.g., Starcraft~\citep{vinyals2019grandmaster}, Dota~\citep{berner2019dota}). 
% Although a lot of environments have pre-defined reward functions, such as the win/loss in board/card games, researchers find proper reward shaping~\citep{hu2020learning} or additional reward design~\citep{faust2019evolving} can further lead to better RL performance.

%\footenote{This is inverse reinforcement learning (IRL). However, we can regard IRL as a sub-domain of IL since they both learn from demonstrations, and IRL still requires to recover a policy.}

Reinforcement learning (RL) has gained encouraging success in various domains, \textit{e.g.}, games~\citep{silver2017mastering,guan2022perfectdou,vinyals2019grandmaster}, robotics~\citep{gu2017deep} and autonomous driving~\citep{pomerleau1991efficient,zhou2020smarts}, which however heavily relies on well-designed reward functions.
Beyond hand-crafting reward functions that are non-trivial, imitation learning (IL) offers a data-driven way to learn behaviors and recover informative rewards from expert demonstrations without access to any explicit reward~\citep{arora2021survey,hussein2017imitation}. 
Recently, visual imitation learning (VIL)~\citep{pathak2018zero,rafailov2021visual} has attracted increasing attention, which aims to learn from high-dimensional visual demonstrations like image sequences or videos. 
Compared with previous IL works tackling low-dimensional inputs, \textit{i.e.} proprioceptive features like positions, velocities, and accelerations~\citep{ho2016generative,fu2017learning,liu2020energy}, VIL is a more general problem in the physical world, such as learning to cook by watching videos. For humans, it is very easy but it remains a critical challenge for AI agents.


Previous approaches apply supervised learning (\textit{i.e.} behavior cloning~\citep{pomerleau1991efficient,pathak2018zero}) or design reward functions~\citep{reddy2019sqil,brantley2019disagreement} to solve VIL problems. 
Among them, supervised methods often require many expert demonstrations and suffer from compounding error~\citep{ross2011reduction}, while the rest tend to design rewards that are too naive to provide appropriate expertise measurements for efficient learning.
Some recent works~\citep{rafailov2021visual,cohen2021imitation,haldar2022watch} choose to directly build on pixel-based RL methods, \textit{i.e.} using an encoder, and learn rewards from the latent space.
These methods inspect the whole image for deriving the rewards, which tend to give only coarse expertise measurements. 
Additionally, they focus on behavior learning, and seldom pay any attention to the explainability of the learned behaviors.


In this work, we argue that the scalar-form reward used in previous works only conveys ``sparse" information of the full image, and hardly measures local expertise, which limits the learning efficiency.
Instead of inducing a scalar reward from the whole image, our intuition is to measure the expertise of different local regions of the given images, or what we call \emph{patches}, and then recover the multi-dimensional rewards, called \emph{patch rewards} accordingly.
Compared with scalar rewards, patch rewards provide a more precise rewarding characterization of visual control tasks, thus supporting efficient IL training and visual explainability of the learned behaviors.
% \textit{e.g.}, which part of the image is good and which is not, or what is the key to resolve the task by expert, \textit{etc}. 


We then propose to achieve more efficient VIL via inferring dense and informative reward signals from images, which also brings better explainability of the learned behaviors.
To achieve this goal, we develop an intuitive and principled approach for VIL, termed Adversarial Imitation Learning with Patch rewards (PatchAIL), which produces patch rewards for agents to learn by comparing local regions of agent image samples with visual demonstrations, and also provides interpretability of learned behaviors.
Also, it utilizes a patch regularization mechanism to employ the patch information and fully stabilize the training.
We visualize the patch rewards induced by our PatchAIL in \fig{fig:intro_heatmaps}.
From the illustration, we can easily interpret where and why agents are rewarded or penalized in these control tasks compared with expert demonstrations without any task prior.
% For example, the Finger Spin task expects the spin of the right body rather than the movement of the Finger; the Hopper Stand task cares more about the movement of the foot than the head and highly punishes the behavior of lying flat; the Cheetah Run and Walker Walk tasks only require the movement of the foot rather than the whole body.
These examples show the friendly explainability of our method, and intuitively tell why the algorithm can work well.


% \begin{figure}[t!]
%     % \vspace{-5pt}
%     \centering
%     \includegraphics[width=\textwidth]{figs/jet_two_rwo-crop.pdf}
%     \vspace{-15pt}
%     \caption{Visualization of patch rewards provided by PatchAIL on Deepmind Control Suite tasks using the final model trained around 200M frames. We map each patch reward back to its corresponding pixels on the middle image of stacked ones. Strikingly, the patch rewards successfully align with the key elements (i.e., robot joints) on both expert and random image samples, indicating where the high rewards (red areas) or low ones (blue areas) come from, compared with the reward on the immutable backgrounds. Figure best viewed on screen.}
%     \label{fig:intro_heatmaps}
%     % \vspace{-15pt}
% \end{figure}

\begin{figure}[t!]
    \vspace{-20pt}
    \centering
    \includegraphics[width=\linewidth]{figs/patchrewardXfeaturemap_four_row-crop.pdf}
    \vspace{-17pt}
    \caption{Visualization of patch rewards by the proposed PatchAIL on seven DeepMind Control Suite tasks. The patch rewards are calculated regarding several stacked frames and are mapped back on each pixel weighted by the spatial attention map.
    We use the final model trained with around 200M frames. Strikingly, the patch rewards align with the movement of key elements (\textit{e.g.}, moving foot, inclined body) on both expert and random samples, indicating where the high rewards (red areas) or low ones (blue areas) come from, compared with the reward on backgrounds. With the patch rewards recovered from expert's visual demonstrations, we can easily reason why and where agents are rewarded or penalized in these tasks compared with expert demonstrations without any task prior. Figure best viewed in color. A corresponding video is provided in the demo page \url{https://sites.google.com/view/patchail/}.}
    \label{fig:intro_heatmaps}
    % \vspace{-8pt}
\end{figure}


We conduct experiments on a wide range of DeepMind Control Suite (DMC)~\citep{tassa2018deepmind} tasks along with several Atari tasks, and find our PatchAIL significantly outperforms all the baseline methods, verifying the merit of our PatchAIL for enhancing the learning efficiency of VIL. 
Moreover, we conduct ablations on the pivotal choices of PatchAIL, showing the key options in PatchAIL such as the number of patches and aggregation function highly impact the learning performance. 
To verify its explainability, we further compare the spatial attention maps of PatchAIL to baseline methods, showing PatchAIL is better at focusing on the correct parts of robot bodies. 
It is hoped that our results could provide some insights for exploiting the rich information in visual demonstrations to benefit VIL and also reveal the potential of using patch-level rewards.
% deepen the understanding of VIL, and shed light on how to make IL more efficient and practical in complex environments.

==> methodology.tex <==

\section{Adversarial Visual Imitation with Patch Rewards}
\label{sec:method}

The proposed Adversarial Imitation Learning with Patch rewards (PatchAIL) method is built upon Adversarial Imitation Learning (AIL) to derive informative and meaningful patch rewards while better explaining expert demonstrations.
%We adopt AIL rather than the classical inverse RL (a.k.a. apprenticeship learning) methods~\citep{abbeel2004apprenticeship,syed2007game}, as it induces the reward from a discriminator in an end-to-end way and better suits image data. 
% Classical inverse reinforcement learning (or known as apprenticeship learning) methods~\citep{abbeel2004apprenticeship,syed2007game} are hard to scale to high-dimensional image data. Therefore, we adopt the paradigm of AIL which induces the reward from a discriminator in an end-to-end way. 
Trained in a GAN-style, the discriminator in AIL works by differentiating the difference between agent samples and expert samples, \textit{i.e.} through a binary-class classification problem that regards the expert data as real (label 1) and the agent data as fake (label 0). 
This strategy works well when learning from the low-level proprioceptive observations, where the reward is given based on the discriminator.
However, this is insufficient when data is videos or image sequences.
With a scalar label to classify and derive the reward simply based on the whole visual area, the images may easily be regarded as far-from-expert due to small noise or changes in local behavior. 
Also, there may be multiple regions of images that affect the rewarding of control tasks, while the discriminator may only focus on insufficient regions that support its overall judgment.
In addition, such scalar rewards are only meaningful for the agent to learn its policy, and they lack explainability for humans to understand where the expertise comes from, such as which parts of the image contribute to higher reward or bring negative effects.
%quanhong: this part should appear in introduction


 %\zw{three points, expand}:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{sensitive to local behavior changes}: the images can be easily regarded as far-from-expert due to small noise or changes in local behavior;
%     \item \textbf{Lost key areas}: judging on the full image area disperses discriminator's attention by only focusing on local evidences that support its overall judgement when multiple regions affects the reward;
%     \item \textbf{Lost key areas}: there may be multiple regions of images that affect the rewarding of control tasks, while the discriminator may only focus on insufficient regions that support its overall judgment;   
%     \item \textbf{Scalar rewards are hard to interpret}: scalar rewards are only meaningful for agent learning its policy, but lack the explainability for humans to understand where the expertise comes from, such as which part of the images contributes to higher reward while others raise negative effects.
% \end{itemize}

%One may argue that the discriminator can measure the expertise based on the latent samples encoded by the encoder trained with pixel-based RL, like in \citep{cohen2021imitation}. This may relieve the sensitivity to local changes, but it is intuitively unreasonable.
In some recent works \citep{cohen2021imitation,rafailov2021visual}, the discriminator measures the expertise based on the latent samples encoded by the encoder trained with pixel-based RL. 
Albeit this may relieve the sensitivity to local changes, it is not intuitively reasonable.
When the discriminator shares the latent space with the critic, the encoder is updated only depending on the critic loss, which is the TD error that is meant to learn correct value prediction depending on the reward obtained from the discriminator.
On the other hand, the discriminator is updated according to the latent space induced by the encoder.
As both modules must be learned from scratch, such interdependence can cause training instability, and deteriorate the attention to key elements related to the expertise. 
Besides, it still lacks explainability due to the scalar label.
%quanhong: I do not see much meaning of discussing this. Usually we tell why we make the right choice rather than why we do not make bad choices


\subsection{From Scalar to Patches}
We make an intuitive and straightforward modification to the classic way of measuring expertise, \textit{i.e.} evaluating different local parts on the given images by replacing the scalar judgment with patch ones. 
By evaluating local parts, on one hand, local changes only affect some of the patches rather than the whole, increasing the robustness of the overall judgment. On the other hand, the discriminator is forced to focus on more areas.
Also, in this way, the classification result and reward on each patch can measure how each part of images contributes the similarity to expert visual demonstrations, which constructs a holistic view for us to understand where the expertise comes from. 

\paragraph{Patch discriminator.}
\begin{wrapfigure}{r}{0.47\textwidth}
  \centering
     \vspace{-23pt}
     \includegraphics[width=0.95\linewidth]{figs/models/patchdisc.pdf}%
     \vspace{-12pt}
     \caption{Illustration of the patch discriminator, where each pixel of the right-side mosaic represents the patch logit corresponding to a local region of the left-side image.}
     \label{fig:patch_discriminator}
     \vspace{-15pt}
\end{wrapfigure}
To implement the idea of the AIL framework, we make the discriminator classify image patches and give \emph{patches of reward} in lieu of \emph{scalar rewards} by learning a single classification result on an image. % $(s, s')\sim\caT$ $(s, s')\sim\caB$
Formally, given a visual demonstration from experts $(s, s')\sim\pi_E$, and the sample from the agent policy $\pi$, we optimize the patch discriminator $\textbf{D}_{P\times P}$ with patch labels:
\begin{equation}\label{eq:disc-loss}
    \begin{aligned}
    \caL(\textbf{D}) = -\bbE_{(s,s)\sim\pi_E}[\log{\textbf{D}_{P\times P}(s,s')}] - \bbE_{(s,s')\sim\pi}[\log{(\textbf{1}_{P\times P}-\textbf{D}_{P\times P}(s,s')})].
    \end{aligned}
\end{equation}
In this formula, the discriminator outputs a matrix of probabilities $\textbf{D}_{P\times P}: \caS \times \caS \rightarrow [0,1]^{P\times P}$, where $P$ is the height/width of each image patch, as illustrated in \fig{fig:patch_discriminator}. 
In other words, the classification loss is computed on each patch logit, rather than on the averaged logit of all patches.
Furthermore, we do not have to maintain an extra encoder for the discriminator and the discriminator learns everything directly from pixels.


\subsection{Learning Framework}
\label{sec:framework}

\paragraph{Reward aggregation.}
\begin{wrapfigure}{r}{0.42\textwidth}
  \centering
    \vspace{-20pt}
     \includegraphics[width=\linewidth]{figs/models/patchail.pdf}
     \vspace{-11pt}
     \caption{The framework of PatchAIL.}
     \label{fig:framework}
     \vspace{-6pt}
\end{wrapfigure}
Generally, the probabilities/logits given by $D$ need to be further transformed by $R=h(D)$ to become a reward function where $h$ transforms probabilities to reward signals, \textit{e.g.} in GAIL~\citep{ho2016generative} $h=\log D$ or $R=-\log (1-D)$, and  $R=\log D-\log (1-D)$ in AIRL~\citep{fu2017learning} and DAC~\citep{kostrikov2018disc}.
In addition, after constructing patch rewards, we need an aggregation function to integrate the global information while deriving scalar signals for training RL agents. Most straightforwardly, one can choose $\texttt{mean}$ as the aggregation operator that evaluates the overall expertise compared to expert visual demonstrations for given image sequences, whilst other kinds of operations can also be adopted. Formally, we can derive the reward function from the discriminator output as
\begin{equation}\label{eq:reward}
    R(s,s') = Aggr(\textbf{R}_{P\times P}(s,s')) = Aggr(h(\textbf{D}_{P\times P}(s,s'))),
\end{equation}
where $Aggr$ aggregates the patch rewards into scalar signals with operators \texttt{mean}, \texttt{max}, \texttt{min} and \texttt{median}. Different aggregation operators can incorporate different inductive biases into the problem and lead to various learning preferences.
% However, we observe that simply compute the patch rewards and aggregate them are not sufficient for reaching a stable performance, as demonstrated in \se{sec:ablation}. We thereby introduce patch regularization taking the advantage of our additional patch rewards.

\paragraph{Patch regularization.} 
By aggregating the patch rewards into scalars, the rich information contained in the patch rewards is lost. In other words, the scalar rewards again only tell the agent about the overall judgment, and the details such as which part of the image is similar to the expert demonstration do not help the learning. To solve this issue, we further propose to regularize the \emph{agent's} patch rewards by comparing them to the \emph{expert's} patch rewards. Intuitively, we not only require the agent to maximize the similarity of the sampled data to the expert but also want the distribution of the agent's patch rewards to be similar to the expert's. To this end, we 
construct a normalized probability mass of a discrete distribution $\Delta(\textbf{D}_{P\times P}(s,s'))$ from the output logits of the patch discriminator (for simplicity we abuse the symbol $\textbf{D}_{P\times P}$ as the unnormalized logits by the discriminator in the following). Formally, we want to maximize the similarity $\texttt{Sim}(s,s')$ to the demonstrations for the observation pair $(s,s')$, where the similarity $\texttt{Sim}(s,s')$ is defined by the nearest statistical distance to the distributions induced by expert samples:
\begin{equation}\label{eq:sim-reg-raw}
\begin{aligned}
    &~~~~~~~\max_{\pi} ~~ \bbE_{(s,s')\sim\pi} [\texttt{Sim}(s,s')] \\
    \texttt{Sim}(s,s') =& \exp{(-\min_{(s_E,s_E')} \ell(\Delta(\textbf{D}_{P\times P}(s,s')), \Delta(\textbf{D}_{P\times P}(s_E,s_E'))))},
\end{aligned}
\end{equation}
where $\ell$ represents some distance metrics.
However, computing \eq{eq:sim-reg-raw} can be time-consuming during training. As a replacement, we choose to compute a simplified similarity $\overline{\texttt{Sim}}(s,s')$ as the distance to the distribution induced by the averaged logits of expert samples instead:
\begin{equation}\label{eq:sim-reg}
    \overline{\texttt{Sim}}(s,s') = \exp{(-\ell(\Delta(\textbf{D}_{P\times P}(s,s')), \Delta(\bbE_{(s_E,s_E')\sim \pi_E}[\textbf{D}_{P\times P}(s_E,s_E'))))}].
\end{equation}
In the experiment we compare these two choices and find the simplified similarity plays a good role in measuring the distance between the expert demonstrations and agent samples.
Particularly, if we instantiate $\ell$ as KL divergence $D_{\text{KL}}$, the similarity is then computed as
\begin{equation}\label{eq:sim-reg-kl}
    \overline{\texttt{Sim}}(s,s') = \exp{(-\sum_{i=1}^P\sum_{j=1}^P \Delta_{i,j}(\textbf{D}_{P\times P}(s,s'))\log\frac{\Delta_{i,j}(\textbf{D}_{P\times P}(s,s'))}{\bbE_{(s_E,s_E')\sim \pi_E}[\Delta_{i,j}(\textbf{D}_{P\times P}(s_E,s_E'))]})},
\end{equation}
where $\Delta_{i,j}$ denotes the probability value of the $(i,j)$-th entry of $\Delta(\textbf{D}_{P\times P})$. The similarity can serve as the regularizer to weigh the aggregated reward signals. 
Considering ways of using the similarity regularizer, we have two variants of the PatchAIL algorithm. 
The first version is named \textit{PatchAIL-W(eight)}, where we take the regularizer as the weighting multiplier on the reward:
\begin{equation}\label{eq:final-reward}
    R(s,s') = \lambda \cdot \overline{\texttt{Sim}}(s,s') \cdot Aggr(h(\textbf{D}_{P\times P}(s,s')))~;
\end{equation}
the other variant is named \textit{PatchAIL-B(onus)}, where the regularizer serves as a bonus term:
\begin{equation}\label{eq:final-reward-aug}
    R(s,s') = \lambda \cdot \overline{\texttt{Sim}}(s,s') + Aggr(h(\textbf{D}_{P\times P}(s,s')))~.
\end{equation}
$\lambda$ is the hyperparameter for balancing the regularization rate.
In our experiments, we find that such a regularization helps stabilize the training procedure on some tasks, as shown in \fig{fig:curve-10}. 

\paragraph{Implementation of the patch discriminator.}
In principle, the architecture of the patch discriminator is an open choice to any good designs to construct patch rewards, such as vision transformer~\citep{isola2017image} (explicitly break input images as patches) or fully-convolution network (FCN)~\citep{long2015fully} (output matrix implicitly mapped back to patches on input images).
In this paper, we choose to implement the patch discriminator as a 4-layer FCN, referring to the one in \citep{zhu2017unpaired}. 
In detail, the discriminator has four convolution layers without MLP connections and keeps the last layer as Sigmoid to give the probabilities of the classification for each patch, where each patch may share some perceptive field with each other. 
The discriminator classifies if each patch is real (\textit{i.e.}, expert) or fake (\textit{i.e.}, non-expert). As a result, we can obtain multi-dimensional rewards by evaluating the expertise of every local region of images.
% Given an image as the input, the discriminator network outputs a feature map whose entries represent different patches of the given image. Different entries may share some receptive fields on the input image. As a result, we can obtain a set of patch rewards evaluating the similarity to the expert demonstration from the patch level.

% \paragraph{Fully convolution network as discriminator.} output as patches.

% \paragraph{Visual transformer as discriminator.} input as patches


\paragraph{Overall algorithm.}
In a nutshell, PatchAIL obtains patch rewards from the patch discriminator, and training agents with reward aggregation and regularization. 
The same as other AIL methods, PatchAIL works with any off-the-shelf pixel-based RL algorithm. In this paper, we choose DrQ-v2~\citep{ye2020mastering} as the underlying component for learning the policy and integrating gradient penalty~\citep{gulrajani2017improved} for training the discriminator. The algorithm is trained under an off-policy style inspired by \citet{kostrikov2018disc}, therefore the agent samples are from the replay buffer $\caB$ and the expert samples are from the demonstration dataset $\caT$.
An overview of the framework is illustrated in \fig{fig:framework}, and the step-by-step algorithm can be found in \ap{ap:algorithm}.


==> paper/motivation_old.tex <==
\section{Visual Imitation on Latent Space with Scalar Reward}
\label{sec:challenge}
Before proposing our solution for VIL, in this section we first investigate two immediate solutions for visual imitation learning from the perspective of \textit{learnability} and \textit{explainablity}.

In the literature of RL, learning policy and value/critic functions from raw pixels usually requires learning an effective image encoder to map images into compact latent representations. 
To this end, many recent works focus on representation learning techniques for pixel-based RL training. 
For instance, \citet{yarats2019improving} trained a regularized autoencoder jointly with the RL agent; % SAC~\citep{haarnoja2017reinforcement}; %SLAC~
\citet{lee2020stochastic} learned a latent world model on top of VAE features and builds a latent value function; \citet{laskin2020curl} optimized contrastive learning objectives to regularize the latent representations; \citet{laskin2020reinforcement,yarats2020image,yarats2021mastering} utilized data augmentation for efficient representation learning. These researchers have also reached a consensus that the policy share the latent representation with the critic, and only the critic loss is used for updating the encoder.
%~\citep{yarats2019improving,yarats2020image,laskin2020reinforcement,laskin2020curl}. 
%, and \citet{yarats2021mastering} further proposed improved techniques for better training efficiency.

For the problem of visual imitation learning (VIL), a straightforward idea is to build existing AIL methods upon the success of pixel-based RL algorithms. In this way, the discriminator takes latent samples and provide scalar logits for corresponding images, resulting in the learning objective:
\begin{equation}\label{eq:latent-ail}
\begin{aligned}
    \caL(D) = -\bbE_{(s,s')\sim\pi}[\log{D(E(s),E(s'))}] - \bbE_{(s,s')\sim\caT}[\log{(1-D(E(s),E(s'))})]~,
    \end{aligned}
\end{equation}
where $E$ is an image encoder.
Technically, there are two options for the learning scheme, shown in \fig{fig:typical_solutions}. A first choice is to construct the discriminator on top of the shared latent space with the policy and the critic (\fig{fig:share-enc}).
This is named \textit{shared-encoder AIL}, which is also exactly the proposal of \citet{cohen2021imitation}. % (except \citet{cohen2021imitation} used a stacked observation but we use observation pairs for the discriminator)
Instead, we can have a second choice, named \textit{independent-encoder AIL}, by letting the discriminator learn its representations (\fig{fig:noshare-enc}) through differentiating the differences between expert images and sampled images.

\paragraph{Learnability.}
From the learning perspective, we first argue that \emph{the discriminator better does not share the representations with the policy/critic}.
Considering when the discriminator shares the latent space with the critic, the update of the encoder only depends on the critic loss, which is the TD error depend on the reward signals in each step obtained from the discriminator; meanwhile, the update of the discriminator also depends on the learning of the latent space incuced by the encoder. Such interdependence can cause training instability when both modules are learned from scratch. 
Additionally, as the shared latent spaces are progressively learned during training, the discriminator will encounter serious distributional shift problems from the latent samples. However, when discriminator learning its representations by itself, \emph{the image classification loss may be sparse to learn a reasonable and compact representations} as well as the critic's encoder does, especially when the agent's samples are quite close to the expert's, increasing the difficulty of training.
% \hypothesis{Conjecture 1}{Discriminator better does not share the representations with the policy/critic.}
\begin{wrapfigure}{r}{0.45\textwidth}
  \centering
    \vspace{-12pt}
     \includegraphics[width=0.88\linewidth]{figs/motivation_10.pdf}
     \vspace{-12pt}
     \caption{Unstable training example with 5 seeds.}
     \label{fig:unstable-training}
     \vspace{-11pt}
\end{wrapfigure}
% \hypothesis{Conjecture 2}{Scalar signals are hard to help the discriminator learn its own representations.}
% in addition, pixel-based RL algorithms always operates from a stack of frames~\citep{mnih2015human} (a stack of 4 frames in Atari experiments and a stack of 3 frames in DMControl for example), aggravating the difficulty and instability on modeling a direct reward function.
We evaluate the two solutions on the Figner-Spin domain to provide empirical evidence for supporting our analysis above, shown in \fig{fig:unstable-training}.
Saliently, we found that they are both unstable in different phases. As expected, independent-encoder AIL tends to fail when the policy behaves near-optimal, indicating that the discriminator may fail to learn a stable and feasible representation through the training procedure. On the contrary, the instability of shared-encoder AIL comes more in the early training stage, although it seems to be more stable at the late stage of the training where the latent representation is almost unchanged. 
% , and we observed it is sensitive to the learning rate of the encoder.


\paragraph{Explainablity.}
\begin{wrapfigure}{r}{0.48\textwidth}
\vspace{-13pt}
\begin{minipage}[b]{0.49\linewidth}
\centering
{\includegraphics[height=0.85\linewidth]{figs/cartpole_gradcam/cartpole_swingup_share_gradcam_random_37_frame0_label-expert.png}
}
{\includegraphics[height=0.85\linewidth]{figs/cartpole_gradcam/cartpole_swingup_share_gradcam_random_37_frame0_label-noexpert.png}
% \vspace{-7pt}
\caption*{(a) Shared-encoder.}
\label{fig:example-suba}
}
\end{minipage}
\begin{minipage}[b]{0.49\linewidth}
\centering
{\includegraphics[height=0.85\linewidth]{figs/cartpole_gradcam/cartpole_swingup_noshare_gradcam_random_37_frame0_label-expert.png}
}
{\includegraphics[height=0.85\linewidth]{figs/cartpole_gradcam/cartpole_swingup_noshare_gradcam_random_37_frame0_label-noexpert.png}
% \vspace{-7pt} 
\caption*{(b) Independent-encoder.}
\label{fig:example-subb}
}
\end{minipage}
\vspace{-14pt}
\caption{Encoder attention maps by GradCAM for expert class (top) and non-expert class (bottom) on an image sample generated by a random policy, where red regions correspond to a high score for the class.}
\vspace{-10pt}
\label{fig:gradcam}
\end{wrapfigure}
Besides the learnability for training, another interesting and important requirement for VIL comes from the visual explanations~\citep{selvaraju2017grad}. A great rewarder learned from the expert data may be able to answer a series of questions, for example, which parts provide the evidence for producing such a low/high reward, or which parts of the image resemble the expert and which parts are not. Algorithms with great explainability / interpretity help people understand the core factors of a task and how an algorithm works, with intuitive guidance to build extensive engineering efforts on resolving the task. For this end, we leverage the off-the-shelf visual explanation tool -- GradCAM~\citep{selvaraju2017grad} to show decision evidence by visualizing the attention map of the encoder when the discriminator predicts rewards on an image sample. The results on the Cartpole-Swingup domain are illustrated in \fig{fig:gradcam}, which is generated by computing the gradients of the score regarding expert/non-expert class on the middle image of stacked ones. 
To our disappointment, we find none of these solutions provide reasonable interprets of the reward inferred. Firstly, 
% by GradCAM, we can only specify the region where the discriminator focuses on, and
\fig{fig:gradcam} simply illustrates that these discriminators judge the class by focusing on a fixed area of the image instead of the robot itself; secondly, \fig{fig:gradcam} only explains where the discriminator is looking at when labeling rewards, yet can hardly tell us why to make such a decision or how to behave like an expert.

As analyzed above, we want to learn an explainable rewarder with decoupled representation from the policy/critic. In this paper, we propose a simple and intuitive method to learn an independent and effective rewarder, which can provide informative reward signals on given images while achieving efficient visual imitation. 
